Vision Transformers with Patch Diversification

Vision transformer has demonstrated promising performance on challenging computer vision tasks. However, directly training the vision transformers may yield unstable and sub-optimal results. Recent works propose to improve the performance of the vision transformers by modifying the transformer structures, e.g., incorporating convolution layers. In contrast, we investigate an orthogonal approach to stabilize the vision transformer training without modifying the networks. We observe the instability of the training can be attributed to the significant similarity across the extracted patch representations. More specifically, for deep vision transformers, the self-attention blocks tend to map different patches into similar latent representations, yielding information loss and performance degradation. To alleviate this problem, in this work, we introduce novel loss functions in vision transformer training to explicitly encourage diversity across patch representations for more discriminative feature extraction. We empirically show that our proposed techniques stabilize the training and allow us to train wider and deeper vision transformers. We further show the diversified features significantly benefit the downstream tasks in transfer learning. For semantic segmentation, we enhance the state-of-the-art (SOTA) results on Cityscapes and ADE20k. Our code is available at https://github.com/ChengyueGongR/PatchVisionTransformer.

==> tex/augmentation.tex <==
\section{Method}

Some recent works (e.g. Transformer in Transformer, Token to Token Transformer, Centroid Transformer) focus on leverage prior knowledge to the transformer model by re-designing the structure.
In this work, however, we argue that the vanilla Transformer structure shown in Figure 1 is powerful enough and focus on let the model converges faster and generalizes better by introducing additional proxy loss (task).


\subsection{Predicting Relative Location for Patches}
An additional head to classify whether two patches are nearby or not at final layer.

\begin{table}[ht]
    \centering
    \begin{tabular}{l|c}
    \hline 
    Model & Top-1 accuracy \\    \hline 
         DEIT Tiny  & 72.2 \\
         w/ predicting location & 72.5 \\
         \hline 
    \end{tabular}
    \caption{Accuracy on ImageNet validation set. Marginal improvement, can not say anything.}
    \label{tab:deit_reproduce}
\end{table}

\subsection{Predicting the Label for Each Patch (Learning to Segment Mixed Image)}

Suppose we have two image-label pairs $(\{x_{0, i}\}, y_0)$ and $(\{x_{1, i}\}, y_1)$, 
we mix the input patches as $\{x_{\text{mix}, i}\}$ where $x_{\text{mix}, i} = \mathbb{I}(\rho < \lambda) x_{0, i} + \mathbb{I}(\rho \geq \lambda) x_{1, i}$ ($\rho$ is sampled from a uniform distribution)
and mix the label  $y_{\text{mix}} = \lambda y_0 + (1 - \lambda) y_1$.
For the last-layer patch $\{h_{\text{mix}, i}\}$ we add an additional patch-level classification loss $\{h_{\text{mix}, i}, y_{\text{mix}, i}\}$. 
In order to save computation cost, we average pooling the patch from the same image and then pass it through the additional patch-level classification loss. 

During evaluation, we do not use the additional proxy loss.
When we mix two images and do not use proxy loss, this is cutmix.

\begin{lstlisting}
patch_loss = 0
for _ in range(len(mask_lst)):
    avgpool_patches = (patches * mask_lst[_]).mean(dim=(2, 3))
    avgpool_logits = F.log_softmax(self.patch_head(avgpool_patches), dim=-1)
    patch_loss += nn.KLDivLoss()(avgpool_logits, target_lst[_])
    
    # patch_loss += nn.KLDivLoss()(avgpool_logits, target_lst[_]) \
    # * target_lst[_].sum() / target_lst[_].size().sum()
\end{lstlisting}

\begin{table}[ht]
    \centering
    \begin{tabular}{l|c|c}
    \hline 
    Model & Top-1 accuracy & Test Loss\\    \hline 
         Cutmix + Mixup (Default)  & 81.8 @ epoch300 & 0.838\\
         Cutmix (reported by DEIT) & 78.7 @ epoch300 & - \\
         Ours (mix two) & 80.8 @ epoch240 & - \\
         \hline 
    \end{tabular}
    \caption{DEIT-Base accuracy on ImageNet validation set. {\color{red} {will be finished tomorrow, together with experiments on DEIT-small.}} }
    \label{tab:deit_reproduce}
\end{table}

\paragraph{How to mix}
Randomly selecting patches or selecting nearby patches like Cutmix.

\begin{table}[ht]
    \centering
    \begin{tabular}{l|c|c}
    \hline 
    Model & Top-1 accuracy & Test Loss\\    \hline 
         Cutmix + Mixup (Default)  & 79.9 @ epoch300 & 0.882 \\
         Randomly Select Patches (mix two) & 80.5 @ epoch300 & 0.827 \\
         Select nearby Patches (mix two) & 80.9 @ epoch300 & 0.809\\
         \hline
         Refine & 81.0 @ epoch300 & - \\
         \hline 
    \end{tabular}
    \caption{DEIT-Small accuracy on ImageNet validation set. `Refine' denotes removing repeat augmentation and adding stronger randaugment.}
    \label{tab:deit_reproduce}
\end{table}

\paragraph{Mixing Rate}
We sample the mixing rate from $\mathrm{Beta}(1, 1)$, and find out this regularization too strong for smaller models while too weak for larger models. 
We need an ablation study here.

\paragraph{Which Layer}
Adding the loss at intermediate layer. 

\paragraph{Over-estimation}
We notice that with our loss, we achieve lower validation loss while the validation accuracy is the same. 
It indicates that some prediction is over-estimated.
Thus, we add an additional reverse KL term in the loss as a regularization term.   {\color{red} {to do...}}

\paragraph{Self-supervision}
The proxy loss can be easily extended to a self-supervised version, in which we mix a bag of images and predicting whether two patches are from a same image.
In this way, 
the analysis of the loss is similar to supervised-LDA. (let's say each image is a topic, each patch is a word, and learning the classification loss is to learn the allocation.)  {\color{red} {future work...}}

\paragraph{Next}
Study whether mixing more images is useful {\color{red} {to do...}}

Without extra data, without extra teacher, we need to beat all the strong CNN models.
Thus, we can try two approaches:
1) increasing the number of patches, 2) using larger models (e.g. VIT-Large).


==> tex/showcase_experiment.tex <==
\lstset{
 columns=fixed,       
 numbers=left,   
 numberstyle=\tiny\color{gray},       
 frame=none,                          
 backgroundcolor=\color[RGB]{245,245,244},  
 keywordstyle=\color[RGB]{40,40,255},  
 numberstyle=\footnotesize\color{darkgray},           
 commentstyle=\it\color[RGB]{0,96,96},  
 stringstyle=\rmfamily\slshape\color[RGB]{128,0,0},  
 showstringspaces=false, 
 language=python,
}

\section{Primal Experiment}
\subsection{Re-Design Self-Attention}
The SoftMax attention in self-attention layer is defined as:
given input $X$, let $K = X W^k$, $Q = X W^q$ and $V = X W^v$, the output $y = \mathrm{SoftMax}(K Q^T / \mathrm{scale}) V$.
The time complexity and FLOPs of the attention is $\mathcal{O}(T^2 N)$ where $T$ is the number of tokens and $N$ is the dimension size.

$X \in R^{[N, D]} -> X^{\mathrm{weight}}_i = X W^{\mathrm{reduce}}_i \in R^{[N, 1]} -> Y = \sum_i X \odot f(X^{\mathrm{weight}}_i)$ where $f$ is stacked MLP with a final sigmoid function and $f(X^{\mathrm{weight}}_i) \in R^{[N, 1]}$.

$x_{i, d} \hookleftarrow f(x_{i, 1:d}) x_{i, d} + x_{i, d}$

$x_{i, d} \hookleftarrow f(x_{1:n, d}) x_{i, d} + x_{i, d}$

Original FLOPs of attention layer in tiny: 350M -> Now: ~20M.

Using attention is not a new idea in computer vision, \citet{hu2018senet, li2019selective} use channel-wise attention to re-weight the importance of each channel.
Inspired by these works, we decompose the SoftMax attention into channel-wise and token/pixel/patch-wise attention. 
The pytorch-style code is:
\begin{lstlisting}
# Linear_1, Linear_2 : linear transform
# Transform_1, Transform_2: 
# stacked full-connected layers with activation functions

# reduce all token for each dimension
x = Linear_1(x) * torch.sigmoid(Transform_1(x.mean(dim=1))) 
# reduce all hidden dimension for each token
x = Linear_2(x) * torch.sigmoid(Transform_2(x.mean(dim=2)))  
\end{lstlisting}
In this way, we re-weight each token and each dimension separately.
The decomposed channel-wise attention is similar to the channel-wise attentions \citep{} which are widely-used in a bunch of computer vision tasks. 
We build two baselines: 1) MLP layers without any attention 2) SoftMax-style self-attention.

\paragraph{Multi-head Patch-wise Attention} 
The information between tokens is only ex-changed in the attention layer. Once we first do a average pooling operation, the expression of the token-level attention is limited. Thus, we create a multi-branch patch-wise attention by sum over several patch-wise attentions with different parameters.

\paragraph{Compare to Efficient Attentions} 
Sparse attention usually has a $\mathcal{O}(T \log(T) N)$ time complexity, and linear attention has a $\mathcal{O}(T N^2)$ complexity. 

First, we would like to see the performance of the decomposed attention.
What is the next step? Further reducing the parameters in MLP layers, or discussing the value of different kind of attention (e.g. If we remove all the attentions, will the performance of the baseline drop a lot? If we only use token-wise attention, will it be much worse than SoftMax-style attention?)

\subsection{LN}
In the original VIT \citep{} and DEIT \citep{}, they use the pre-LayerNorm \citep{} as:

\begin{lstlisting}
x = x + self.drop_path(self.attn(self.norm1(x)))
x = x + self.drop_path(self.mlp(self.norm2(x)))
\end{lstlisting}

% In NLP community, people has already aware that 1)
% In the following, we test some cases to see whether they are important for image transformer. 
We use the open-source code of DEIT \footnote{\url{https://github.com/rwightman/pytorch-image-models/blob/master/timm/models/vision_transformer.py}}. 
% and the source file of the transformer module is 

\subsection{Relative Position Information}
The relative position information can be added into the attention or outside.  

We test three module, 

1) Relative Positional Embedding \citep{}:
\begin{lstlisting}
self.remb = nn.Parameter(torch.randn([197, embed_dim//num_heads,197])*0.02)
trunc_normal_(self.remb,std=.02)
                
rpos=q.permute(2,0,1,3).reshape(N,B*self.num_heads,C//self.num_heads)@self.remb
rpos=rpos.reshape(N,B,-1,N)
attn=(q@k.transpose(-2,-1)+ rpos.permute(1,2,0,3))*self.scale
\end{lstlisting}
2) MLP as an expansion block: change MLP Layer from Linear(192, 768)-Linear(768, 192) to MLP(192, 768)-Conv(input=192,output=192,groups=192)-MLP(192, 768). 

3) Adding a channel-wise conv layer before MLP layer to force local attention for the 14x14 patches.
We change the attention to 
\begin{lstlisting}
self.conv = torch.nn.Conv2d(in_channels=dim, \ 
out_channels=dim, kernel_size=3, groups=dim, padding=1)

x = x + self.drop_path(self.attn(self.norm1(x)))
batch_size, hidden, patch_length = x.shape[0], x.shape[-1], 224 // 16
x[:, 1:, :] = x[:, 1:, :] + self.conv(x[:, 1:, :].transpose(1, 2) \
.reshape(batch_size, hidden, patch_length, patch_length))\
.reshape(batch_size, hidden, patch_length*patch_length).transpose(1, 2)
x = x + self.drop_path(self.mlp(self.norm2(x)))
\end{lstlisting}

\begin{table}[h]
    \centering
    \begin{tabular}{cccc}
        \hline
        Model & Params & Additional FLOPs & Accuracy \\
        \hline
        Tiny DEIT & 5.7M & 0M & 72.2\% \\
        \hline
        + Relative Embedding  & 8.2M & 178M & 72.3\% \\
        + Conv in MLP  & 5.7M & 16M & 72.5\% \\
        + Conv outside MLP  & 5.7M & 4M & \bf{73.6\%} \\
        \hline
    \end{tabular}
    \caption{ImageNet.}
    \label{tab:none}
\end{table}


\begin{figure}[ht]
    \centering
    \begin{tabular}{c}
    \includegraphics[width=0.4\textwidth]{figures/vit_pos_emb.pdf} 
    \end{tabular}
    \label{fig:vit_base}
    \caption{Introducing learnanble positional embeddings.}
\end{figure}



\subsection{LayerNorm}
In NLP, the pre LayerNorm \citep{xiong2020layer} can accelerate the training. However, the post norm (which is used in the original transformer) usually achieves better result. We have a test on it
1) post LN :
\begin{lstlisting}
x = self.norm1(x + self.drop_path(self.attn(x)))
x = self.norm2(x + self.drop_path(self.mlp(x)))
\end{lstlisting}

2) additional LN normalization:
\begin{lstlisting}
attn_x = x + self.drop_path(self.attn(self.norm1(x)))
x = attn_x + self.drop_path(self.mlp(self.norm2(attn_x)))
x = self.norm3(x + attn_x)
\end{lstlisting}

\begin{table}[h]
    \centering
    \begin{tabular}{cccc}
        \hline
        Model & Params & Additional FLOPs & Accuracy \\
        \hline
        Tiny DEIT & 5.7M & 0M & 72.2\% \\
        \hline
        Post LN  & 5.7M & 0M & 70.8\% \\
        + Additional LN  & 5.7M & ~0M & \bf{72.4\%} \\
        \hline
    \end{tabular}
    \caption{ImageNet.}
    \label{tab:none}
\end{table}

\subsection{MLP}
Is where to put the MLP and to put how many MLP important?
We use a weight-shared MLP:

\begin{lstlisting}
x = x + self.drop_path(self.attn(self.norm1(x)))
for mlp_index in range(num_mlp):
    x = x + self.drop_path(self.mlp(self.norm2(x))) /n
\end{lstlisting}, 

and a weight-unshared MLP:
\begin{lstlisting}
x = x + self.drop_path(self.attn(self.norm1(x)))
for mlp_index in range(num_mlp):
    x = x + self.drop_path(self.mlp[mlp_index](self.norm2[mlp_index](x))) / n
\end{lstlisting},
to see whether there is difference. Notice that the original MLP(dim-hidden-dim) increase the hidden size to $4\times$dimension size, we decrease the MLP hidden size to make the number of parameters the same.

We set the number of layer to 2 to do a test.
\begin{table}[h]
    \centering
    \begin{tabular}{cccc}
        \hline
        Model & Params & Additional FLOPs & Accuracy \\
        \hline
        Tiny DEIT & 5.7M & 0M & 72.2\% \\
        \hline
        Shared MLP  & 5.7M & 500M & 72.4\% \\
        Unshared MLP  & 5.7M & 0M & \bf{72.5\%} \\
        \hline
    \end{tabular}
    \caption{ImageNet.}
    \label{tab:none}
\end{table}

\subsection{Initialization and Optimization}
We test Fixup and its followup \citep{huang2020improving}, it does not have an impact on the final result. 

\subsection{Hand-Crafted and NAS}
We combine these features to design a new network structure:
\begin{lstlisting}
batch_size, hidden, patch_length = x.shape[0], x.shape[-1], 224 // 16
x[:, 1:, :] += Conv(x[:, 1:, :])
x = self.norm1(x)
x = x + 1. / 2 * self.drop_path(self.mlp1(x))

x = self.norm2(x)
x = x + self.drop_path(self.attn(x)) 

x[:, 1:, :] += Conv(x[:, 1:, :])
x = self.norm3(x)
x = x + 1. / 2 * self.drop_path(self.mlp(x))
x = self.norm4(x)
\end{lstlisting}

We also use a DARTs-like NAS method to do a search. Note that in the search space, when we decide whether to use a module (e.g. LayerNorm, Conv) or Identity, we add a penalty on the Identity operator to avoid degenerate during searching.

\textbf{We not only achieve much better results, but also accelerate the training by a large margin (e.g. Training with 20 epochs on Tiny-DEIT, we improve the 25\% top-1 accuracy baseline to 54\%).}

\begin{table}[h]
    \centering
    \begin{tabular}{cccc}
        \hline
        Model & Params & Additional FLOPs & Accuracy \\
        \hline
        Tiny DEIT & 5.7M & 0M & 72.2\% \\
        Human-Design  & 5.7M & 8M & \bf{74.2\%} (not finished) \\
        NAS  & 5.7M & 0M & \bf{-} \\
        \hline
        Small DEIT & 16.8M & 0M & 79.9\% \\
        Human-Design  & 16.8M & 16M & \bf{81.1\%} (not finished) \\
        NAS  & 5.7M & 0M & \bf{-} \\
        \hline
    \end{tabular}
    \caption{ImageNet. \textbf{Our result is even better than the DEIT with teacher model.}}
    \label{tab:none}
\end{table}


\subsection{More...}
The next step is either designing a mobile-version or designing the attention module.
Let us make a short version as a workshop paper first.

==> tex/vit.tex <==
\section{Vision Transformers}

\begin{figure}[ht]
    \centering
    \begin{tabular}{c}
    \includegraphics[width=0.4\textwidth]{figures/vit_base.pdf} 
    \end{tabular}
    \label{fig:vit_base}
    \caption{Overview of basic vision transformer.}
\end{figure}


